M3SciQA: A Multi-Modal Multi-Document Scientific QA Benchmark for Evaluating Foundation Models

Existing benchmarks for evaluating foundation models mainly focus on single-document, text-only tasks. However, they often fail to fully capture the complexity of research workflows, which typically involve interpreting non-textual data and gathering information across multiple documents. To address this gap, we introduce M3SciQA, a multi-modal, multi-document scientific question answering benchmark designed for a more comprehensive evaluation of foundation models. M3SciQA consists of 1,452 expert-annotated questions spanning 70 natural language processing paper clusters, where each cluster represents a primary paper along with all its cited documents, mirroring the workflow of comprehending a single paper by requiring multi-modal and multi-document data. With M3SciQA, we conduct a comprehensive evaluation of 18 foundation models. Our results indicate that current foundation models still significantly underperform compared to human experts in multi-modal information retrieval and in reasoning across multiple scientific documents. Additionally, we explore the implications of these findings for the future advancement of applying foundation models in multi-modal scientific literature analysis.

==> main/ethics.tex <==
% \section*{Ethics Statement}
% This is the ethics statement.

% 1. address future data contamination

==> table_tex/app_bootstrap.tex <==
\begin{table*}[!h]
\centering
\small
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\bb{Model} 
& Llama
& Mistral
& DBRX
& Command R+
& GPT-4
& GPT-3.5
& Gemini
& Sonnet
& Opus
\\ \midrule
Llama-2-70B & - & 0.5809 & 0.5791 & 0.9994 & 0.9487 & 0.9749 & 0.9227 & 0.8960 & 0.8496\\
Mistral-7B & - & - & 0.0523 & 1.0000 & 0.9946 & 0.9959 & 0.891 & 0.9871 & 0.9685\\
DBRX & - & - & - & 0.9994 & 0.9622 & 0.9815 & 0.8826 & 0.9189 & 0.8906\\
$^\dagger$Command R+ & - & - & - & - & 0.0811 & 0.1302 & 0.0016 & 0.0602 & 0.0272\\
\midrule
$^\dagger$GPT-4 & - & - & - & - & - & 0.5866 & 0.0557 & 0.3952 & 0.2683\\
$^\dagger$GPT-3.5 & - & - & - & - & - & - & 0.034 & 0.3077 & 0.2327\\
$^\dagger$Gemini-Pro-1.0 & - & - & - & - & - & - & - & 0.8696 & 0.8363\\
$^\dagger$Claude-3-Sonnet & - & - & - & - & - & - & - &- & 0.3905\\
$^\dagger$Claude-3-Opus & - & - & - & - & - & - & - &- & -\\
\bottomrule
\end{tabular}%

\caption{Pairwise {bootstrapping test} over \emph{test} set result. Each entry represents the probability that model in the corresponding \bb{column} performs worse than model in the corresponding \bb{row}. The higher the value, the more likely that the \bb{row} model outperforms the \bb{column} model.}
\label{tab:bootstrap}
\end{table*}

==> table_tex/detail_3_settings_gpt.tex <==
\begin{table}[!t]
  \centering
  \small
  \begin{tabular}{lccc}
    \toprule
    \bb{Model} & 
    \textbf{Title-Only} & 
    \textbf{\begin{tabular}[c]{@{}c@{}}Retrieval \\($k=3$)\end{tabular}} & 
    \textbf{Oracle} \\
    \midrule
    Mistral & 23.75 & & 25.00\\
    Mixtral & 14.25 & & \\
    DBRX & & 19.75 & 47.25 \\
    Command R+ & & 29.25 & 56.50\\
    PaLM-2 & & & 55.50\\
    \addlinespace[0.2em]\hdashline\addlinespace[0.2em]
    GPT-4 & 32.50 & 25.25 & 63.25\\
    GPT-3.5 & 22.75 & 26.00 & 60.75\\
    \bottomrule
  \end{tabular}
  \caption{LLM-based accuracy score for the \emph{title-only}, \emph{retrieval}, and \emph{oracle} settings, based on 200 randomly sampled questions from \emph{test} set of \data. \ziyao{precision recall: add finding 0.2525 < 0.6325*0.48; at the same time talk about percentage @ 3 add up to more than 50\%}}
  \label{tab:detail_3_settings_gpt}
\end{table}

==> table_tex/detail_baseline.tex <==
\begin{table*}[hbt!]
\centering
\small
\begin{tabular}{@{}lccccccccc@{}}
\toprule
\textbf{} & \textbf{\begin{tabular}[c]{@{}c@{}}Val\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}Test\end{tabular} } 
& \textbf{\begin{tabular}[c]{@{}c@{}}CU\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}II\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}RDI\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}MA\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}CA\end{tabular}} 
\\
& (568) 
& (1,000) 
& (207)
& (204)
& (194) 
& (202) 
& (193) 
\\ \midrule

Random Choice & 14.44 & 16.05 & 15.72 & 16.13 & 16.02 & 16.41 & 16.05    \\ 
\midrule
\multicolumn{8}{c}{\textbf{Large Language Models (LLMs): Text as Input}} \\ 
\midrule
%
Llama-2-13B  & - & 20.52 & 19.48 & 13.56 & 17.14 & 18.75 & 25.00    \\

%
Mistral-7B  & 20.55 & 19.16 & 22.50 & 14.85 &  21.28 & 20.30 & 16.93    \\
%
Mixtral-8x7B \href{https://huggingface.co/docs/transformers/en/model_doc/mixtral}{link}  & 23.06 & 20.40 & 17.48 & 22.39 & 21.13& 18.41 & 22.87   \\

PaLM-2 & - & 52.25 & 60.24 & 56.17 & 44.65 & 45.45 & 52.20\\
StripedHyena-Nous-7B & - & 43.38 & 43.85 & 46.24&36.09&48.26&45.24\\
%
Flan-UL2 \href{https://huggingface.co/google/flan-ul2}{link}  & - & - & - & - & -& - & -    \\
%
Tulu-7B \href{https://huggingface.co/allenai/tulu-7b}{link}  & - & - & - & - & -& - & -    \\
%
ChatGLM2-6B \href{https://github.com/THUDM/ChatGLM2-6B/blob/main/README_EN.md}{link}  & - & - & - & - & -& - & -    \\
%
Alpaca-7B \href{https://github.com/tatsu-lab/stanford_alpaca}{link}  & - & - & - & - & -& - & -   \\
%
Vicuna-13B \href{https://huggingface.co/lmsys/vicuna-13b-v1.3}{link}  & - & - & - & - & -& - & -    \\
%
GPT-JT-6B \href{https://huggingface.co/togethercomputer/GPT-JT-6B-v1}{link}  & - & - & - & - & -& - & -   \\
%
Dolly-v2-12B \href{https://huggingface.co/databricks/dolly-v2-12b}{link}  & - & - & - & - & -& - & -    \\
%
T0 \href{https://huggingface.co/bigscience/T0}{link}  & - & - & - & - & -& - & -    \\
%
Gemma  \href{https://blog.google/technology/developers/gemma-open-models/}{link} & - & - & - & - & -& - & -    \\

\addlinespace[0.1em]\hdashline\addlinespace[0.1em]
%
\rowcolor{lavender} GPT-4   &  &  &  &  & &  &     \\
\quad \quad title only  & 69.66 & 72.50 & 77.20 & 72.54 & 62.88 &  65.35  & 77.20 \\
\quad \quad Retrieval (306) & 62.74 & - & 71.3 (val) & 75.41 (val) & 82.45 (val) & 31.88 (val) & 76.27 (val) & 53.33 (val)\\
\quad \quad Oracle   & 75.53 & 75.40 & 91.30 & 72.06 & 57.73 &  72.27  & 82.90 \\

%
\rowcolor{lavender} GPT-3.5-turbo   &  &  &  &  &  &  &     \\
\quad \quad w/ RAG    & 63.89 & 65.50 & 78.74 & 64.22 & 56.19 & 59.90  &  67.88 \\
\quad \quad w/o RAG   & 51.25 & 54.54 & 72.46 & 51.47 & 36.65 & 48.00 & 63.16    \\

%
\rowcolor{lavender} Gemini-Pro-1.0  &  &  &  &  &  &  &  \\
\quad \quad w/ RAG   & 41.07 & 41.70 & 47.83 & 34.80 & 28.35 & 49.01  & 51.30 \\
\quad \quad w/o RAG   & 56.51 & 59.54 & 73.43 & 63.73 & 34.04 &  57.21 & 67.02 \\
%
 Claude-3-Haiku  &  &  &  & & &  &     \\

%
 Claude-3-Sonnet  &  &  &  &  & &  &     \\

Claude-3-Opus  &  &  &  &  & &  &     \\


\bottomrule
\end{tabular}%
\caption{Overall results of different models on the \data \textbf{validation} and \textbf{test set}. The best-performing model in each category is \textbf{in-bold}, and the second best is {\ul{underlined}}.}
\label{tab:detail}
\end{table*}




% \begin{table*}[hbt!]
% \centering
% \small
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{} & \textbf{\begin{tabular}[c]{@{}c@{}} Total\end{tabular}} 
% & \textbf{\begin{tabular}[c]{@{}c@{}}CU\end{tabular}} 
% & \textbf{\begin{tabular}[c]{@{}c@{}}II\end{tabular}} 
% & \textbf{\begin{tabular}[c]{@{}c@{}}RDI\end{tabular}}
% & \textbf{\begin{tabular}[c]{@{}c@{}}MA\end{tabular}} 
% & \textbf{\begin{tabular}[c]{@{}c@{}}CA\end{tabular}} 
% \\
% & (963) 
% & (199)
% & (197)
% & (208) 
% & (184) 
% & (175) 
% \\ \midrule

% GPT-4 \\
% \quad \quad title only & 36.34 & 51.26 & 35.03 & 23.56 & 36.69 & 35.43 \\
% \quad \quad Retrieval & 52.50 & 57.14 & 82.35 & 38.89 & 30.77 & 50.00\\
% \quad \quad Oracle & 73.62 & 90.45 & 65.99 & 60.58 & 71.74 & 80.57\\

% GPT-3.5-turbo \\
% \quad \quad title only & 31.36 & 49.25 &28.43 & 22.60 & 24.46 &32.00 \\

% %
% Gemini-Pro-1.0  &  &  &  &  &  &  &  \\
% \quad \quad title only & 51.58 &  68.53 & 54.82 & 33.66 & 46.41 & 58.72 \\
% % \quad \quad Oracle & 33.71 & 44.72 & 37.06 & 22.60 & 32.79 & 41.95 \\
% Claude-3-Opus  &  &  &  &  & &       \\
% \quad \quad title-only (350 examples) & 18.87 & 14.49 & 15.28 & 19.77 & 11.76 & 13.33\\
% \quad \quad Oracle & 72.24 & 85.71 & 65.00 & 57.69 & 80.95 & 71.43\\


% \bottomrule
% \end{tabular}%
% \caption{Overall results of different models on the \data \textbf{validation} and \textbf{test set}. The best-performing model in each category is \textbf{in-bold}, and the second best is {\ul{underlined}}.}
% \label{tab:detail}
% \end{table*}

==> table_tex/detail_gpt_acc.tex <==
\begin{table*}[hbt!]
\centering
\small
\begin{tabular}{@{}lccccccccc@{}}
\toprule
{Model} 
& \textbf{\begin{tabular}[c]{@{}c@{}}Val\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}Test\end{tabular} } 
& \textbf{\begin{tabular}[c]{@{}c@{}}CU\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}II\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}RDI\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}MA\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}CA\end{tabular}} 
\\
& (452) 
& (1,000) 
& (193)
& (193)
& (208) 
& (217) 
& (189) 
\\ \midrule

Expert Performance  & - & - & - & - & -& - & -    \\ 
\midrule
\multicolumn{8}{c}{\emph{Large Language Models (LLMs): Text as Input}} \\ 
\midrule
%
Llama-2-70B  \cite{touvron2023llama}   \\
%
Mistral-7B \cite{jiang2023mistral} & & 21.91 & 22.02 & 22.22 & 14.20 & 21.43 & 30.00\\
%
Mixtral-8x7B  \cite{jiang2024mixtral} \\
%
PaLM-2 \cite{anil2023palm} & 13.72 & 14.90 & 20.21 & 12.69 & 11.78 & 14.29 & 15.87 \\

Tulu-2-70B   & - & - & - & - & -& - & -    \\

Gemma  & - & - & - & - & -& - & -    \\
%
DBRX \cite{DBRX} & & 45.45 & 50.52 & 48.45 & 27.64 & 48.16 & 53.70 \\
%
Command R+ \cite{commandR+} & 51.30 & 56.40 & 63.21 & 56.74 & 48.08 & 54.38 & 56.40\\

\addlinespace[0.1em]\hdashline\addlinespace[0.1em]
%
GPT-4 \cite{openai2024gpt4} \\
\quad \quad title only  & 15.04 & 20.50 & 16.32 & 24.09 & 1.44 & 18.43 & 17.72\\
\quad \quad Retrieval &  &  &  &  & &  &\\
\quad \quad Oracle & 74.12 & 75.80 & 75.91 & 63.47 & 59.13& 69.12 &67.20 \\
% 
GPT-3.5   &  &  &  &  & &  &     \\
\quad \quad title only & 25.00 & 29.30 & 20.21 & 28.76 & 5.53 & 24.65 & 28.57 \\
\quad \quad Retrieval  &  & \\
\quad \quad Oracle &   & 59.90 & 65.28 & 58.55 & 49.28 & 60.14 & 67.20  \\

\bottomrule
\end{tabular}%

\caption{\hl{GPT-based accuracy score} on \emph{validation} and \emph{test} set of \data. The best-performing model in each category is \textbf{in-bold}, and the second best is {\ul{underlined}}. Reasoning types: CU: conceptual understanding, II: implications and Inferences, RDI: results and data interpretation, MA: methodological analysis, CA: critical analysis.}
\label{tab:detail_gpt_based}
\end{table*}





==> table_tex/detail_multi_metrics.tex <==
\begin{table*}[hbt!]
\centering
\small
\begin{tabular}{@{}lccccccccc@{}}
\toprule
{Model} 
& \textbf{\begin{tabular}[c]{@{}c@{}}ROUGE-1\end{tabular} } 
& \textbf{\begin{tabular}[c]{@{}c@{}}ROUGE-2\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}ROUGE-l\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}BERTScore \\ Precision\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}BERTScore \\ Recall\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}A3CU\\F1\end{tabular}} 
\\ \midrule

%
Llama-2-70B   & - & - & - & -& - & - \\
%
Mistral-7B & 0.154 & 0.077 & 0.124 & - & - & 0.107\\
%
Mixtral-8x7B   & 0.055 & 0.019 & 0.045 & - & & 0.104\\
%
PaLM-2 & 0.197 & 0.095 & 0.157 & - & - & 0.113\\
%
Tulu-2-70B     & - & - & -& - & -    \\
%
Gemma  & -  & - & - & - & - & -    \\
%
DBRX & 0.155 & 0.075 & 0.122 & - & - & 0.111\\
%
$^\dagger$Command R+ & 0.205 & 0.079 & 0.176 & -& - & 0.115\\
%
\addlinespace[0.1em]\hdashline\addlinespace[0.1em]
%
$^\dagger$GPT-4  & 0.237 & 0.127 & 0.202 & 0.858 & 0.851 & 0.158\\
%
$^\dagger$GPT-3.5  & 0.208 & 0.101 & 0.171 & 0.851 & 0.842 & 0.118 \\
%
$^\dagger$Gemini-Pro-1.0  & 0.179 & 0.090 & 0.151 & - & - & 0.112\\
%
$^\dagger$Claude-3-Haiku & 0.176 & 0.090 & 0.143 & - & - & 0.118\\ 
%
$^\dagger$Claude-3-Sonnet  & 0.184 & 0.086 & 0.144 & - & - & 0.111\\
%
$^\dagger$Claude-3-Opus& 0.171 & 0.834 & 0.135 & - & - & 0.121\\
\bottomrule
\end{tabular}%

\caption{\hl{Different metrics} on \emph{test} set of \data in \emph{retrieval} setting from GPT-4V(ision)'s retrieval. The best-performing model in each category is \textbf{in-bold}, and the second best is {\ul{underlined}}. Reasoning types: CU: conceptual understanding, II: implications and Inferences, RDI: results and data interpretation, MA: methodological analysis, CA: critical analysis.}
\label{tab:detail_gpt_based}
\end{table*}





==> table_tex/different_retrieval_setting.tex <==
\begin{table}[!t]
  \centering
  \small
  \begin{tabular}{lcc}
    \toprule
    \textbf{Setting} & \textbf{Mistral 7B} & \textbf{GPT-4} \\
    \midrule
    title-only & 25.00 & 20.50 \\
    $k=1$ & 11.50 & 21.50 \\
    $k=2$ & 17.50 & 24.50 \\
    $k=3$ & 19.50 & 30.50 \\
    $k=4$ & 18.00 & 24.50 \\
    $k=5$ & 20.50 & 23.00 \\
    \midrule
    Oracle & 44.50 & 61.50\\    
    \bottomrule
  \end{tabular}
  \caption{Results of detail question under different retrieval setting on the 100 randomly sampled questions from \emph{test} set of \data. \chuhan{this can be drawn in a graph}}
  \label{tab:different_retrieval_setting}
\end{table}

==> table_tex/gpt_embedding_mrr.tex <==
\begin{table}[!t]
  \centering
  \small
  \begin{tabular}{lcc}
    \toprule
    \textbf{Embedding Model} & \textbf{MRR (Val)} & \textbf{MRR (Test)} \\
    \midrule
    % GPT-4V(ision)   & 0.400 \\
    GPT-4 Omni  & 0.488 & 0.500 \\
    GPT-4V(ision) & 0.404 & 0.400 \\
    \addlinespace[0.2em]\hdashline\addlinespace[0.2em]
    \texttt{text-embedding-ada-002} & 0.206 & 0.182 \\
    \texttt{text-embedding-3-small} & 0.236 & 0.225 \\
    \texttt{text-embedding-3-large} & 0.310 & 0.310 \\
    % \midrule
    % GPT-4V(ision)   & 0.400 \\
    % Claude-3-Sonnet & 0.379\\
    % Claude-3-Opus & 0.326\\
    \bottomrule
  \end{tabular}
  \caption{Comparison of MRR on the \emph{validation} and \emph{test} sets among various OpenAI textual embedding models, including GPT-4 Omni and GPT-4V(ision).}
  \label{tab:gpt_embedding_mrr}
\end{table}

==> table_tex/main_reasoning_table.tex <==
\begin{table*}[!t]
  \centering
  \small
  \begin{tabular}{cl}
    \toprule
    \textbf{\begin{tabular}[c]{@{}c@{}}Question Types\end{tabular}}& 
    \textbf{\begin{tabular}[c]{@{}c@{}}Reasoning Types\end{tabular}}\\
    \midrule
    \bb{Locality-Specific Reasoning} 
    & \begin{tabular}[c]{@{}l@{}}Comparison, Data Extraction, Location, Visual Understanding\end{tabular}\\
    \addlinespace[0.2em]\hdashline\addlinespace[0.2em]
    \bb{Detail-Specific Reasoning} 
    & \begin{tabular}[c]{@{}l@{}}Conceptual Understanding, Methodological Analysis, \\ Results and Data Interpretation, Implications and Inferences, Critical Analysis\end{tabular}\\
    \bottomrule
  \end{tabular}
  \caption{Reasoning types for locality-specific questions and detail-specific questions. Definitions and examples can be found in Table \ref{tab:locality_reasoning} and Table \ref{tab:detail_reasoning_definition} in Appendix \ref{appendix:data-collection}}
  % \label{tab:locality_error_analysis}
\end{table*}

==> table_tex/reasoning_example.tex <==
\begin{table*}[!t]
\centering
\small
\renewcommand\tabcolsep{1.0pt} % column space
\begin{tabular}{cp{11.5cm}}
    \toprule
    \textbf{Locality Reasoning} & \textbf{Description} \\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Comparison \\ \centering(\text{38.71\%})}}
    &  It focuses on evaluating and contrasting information presented in tables, figures, or other data formats. To answer questions of this type, one must analyze and compare specific subjects or variables within the given data set. \emph{Example: Which model shown in the figure consistently better than MPT-7B-Instruct but consistently worse than LLaMA-30B}. \\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Data Extraction \\ \centering(\text{33.47\%})}}
    &  It directly retrieves specific information from table or figure. This approach focuses on pinpointing exact data points or details. \emph{Example: Which model demonstrates score of 21.073 in 10-shot prompting}\\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Location  \\ \centering(\text{15.29\%})}}
    &  It centers on pinpointing spatial or positional information from table or figure. This involves identifying either relative or absolute locations, like the placement of items in a figure or row information in a table. \emph{Example: Which dataset lies on the second left in the figure?}\\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Visual Understanding \\ \centering(\text{12.53\%})}}
    & It emphasizes on the visual information from the figure such as colors, shapes, and marker types. This approach involves closely analyzing these visual cues to extract relevant information. \emph{Example: What is the model represented with a blue line in the figure?}\\
    \toprule
    \textbf{Detail Reasoning} & \textbf{Description} \\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Conceptual Understanding \\ \centering(\text{21.62\%})}}
    &  Evaluate knowledge of essential concepts, basic theories, and critical definitions related to the subject. \emph{Example: What does the hypernetwork in the proposed Hyperdecoders approach generate?}\\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Methodological Analysis \\ \centering(\text{21.01\%})}}
    & Examine and assess the research methodologies and experimental frameworks employed in studies, with an emphasis on their efficacy and constraints. \emph{Example: What potential application of the Hyperdecoder approach is suggested by its performance on long-context out-of-domain datasets in the MRQA evaluation?} \\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Results and Data Interpretation \\ \centering(\text{19.49\%})}}
    & Analyze statistical data, graphs, and tables, focusing on deriving significant insights and conclusions from quantitative and visual information. \emph{Example: In the experimental results for the GLUE benchmark using $T5_{large}$ v1.1 + LM as the underlying model, which model configuration achieved the highest average score across tasks?} \\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Implications and Inferences \\ \centering(\text{19.21\%})}}
    & Infer wider implications and practical uses of study outcomes, concentrating on the extensive impact and prospective significance of the results. \emph{Example: What is the primary purpose of introducing domain prompts in ELLE?}\\
    \midrule
    \multirow{3}{*}{\parbox{4cm}{\centering Critical Analysis \\ \centering(\text{18.66\%})}}
    & Assess the study’s reasoning, robustness of evidence, and validity of conclusions critically, with a focus on logical consistency and the support of empirical data. \emph{Example: What is the primary goal of ELLE as described in the paper?} \\
    \bottomrule
\end{tabular}
\caption{Definitions and proportions of reasoning categories in \data.}
\label{tab:reasoning definition}
\end{table*}
